Gradients as a Measure of Uncertainty in Neural Networks

Despite tremendous success of modern neural networks, they are known to be overconfident even when the model encounters inputs with unfamiliar conditions. Detecting such inputs is vital to preventing models from making naive predictions that may jeopardize real-world applications of neural networks. In this paper, we address the challenging problem of devising a simple yet effective measure of uncertainty in deep neural networks. Specifically, we propose to utilize backpropagated gradients to quantify the uncertainty of trained models. Gradients depict the required amount of change for a model to properly represent given inputs, thus providing a valuable insight into how familiar and certain the model is regarding the inputs. We demonstrate the effectiveness of gradients as a measure of model uncertainty in applications of detecting unfamiliar inputs, including out-of-distribution and corrupted samples. We show that our gradient-based method outperforms state-of-the-art methods by up to 4.8% of AUROC score in out-of-distribution detection and 35.7% in corrupted input detection.

==> cover.tex <==
\pagestyle{empty}
\begin{document}
\twocolumn[{%
\vspace{30mm}
%\renewcommand\twocolumn[1][]{#1}%
{ \large
\begin{itemize}[leftmargin=2.5cm, align=parleft, labelsep=2cm, itemsep=4ex,]

\item[\textbf{Citation}]{G. Kwon, M. Prabhushankar, D. Temel, and G. AlRegib, “Novelty Detection Through Model-Based Characterization of Neural Networks,” 2020 27th \textit{IEEE International Conference on Image Processing (ICIP)}, Abu Dhabi, United Arab Emirates (UAE), 2020.}

\item[\textbf{Review}]{Date of Publication: October 25, 2020}

\item[\textbf{Codes}]{\url{https://github.com/olivesgatech/gradcon-anomaly}}

\item[\textbf{Bib}]  {@inproceedings\{kwon2020novelty,\\
    title=\{Novelty Detection Through Model-Based Characterization of Neural Networks\},\\
    author=\{Kwon, Gukyeong and Prabhushankar, Mohit and Temel, Dogancan and AlRegib, Ghassan\},\\
    booktitle=\{2020 IEEE International Conference on Image Processing (ICIP)\},\\
    year=\{2020\}\}}

\item[\textbf{Copyright}]{\textcopyright 2020 IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes,
creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component
of this work in other works. }

\item[\textbf{Contact}]{
\{gukyeong.kwon, mohit.p, cantemel, alregib\}@gatech.edu\\
\url{https://ghassanalregib.info/}\\}
\end{itemize}
}}]
% \thispagestyle{empty}
\newpage
\clearpage
\setcounter{page}{1}

% Title.
% ———
\title{Novelty Detection through Model-Based\\ Characterization of Neural Networks}
